CSV: Image Quality Assessment Based on Color, Structure, and Visual System

This paper presents a full-reference image quality estimator based on color, structure, and visual system characteristics denoted as CSV. In contrast to the majority of existing methods, we quantify perceptual color degradations rather than absolute pixel-wise changes. We use the CIEDE2000 color difference formulation to quantify low-level color degradations and the Earth Mover's Distance between color name descriptors to measure significant color degradations. In addition to the perceptual color difference, CSV also contains structural and perceptual differences. Structural feature maps are obtained by mean subtraction and divisive normalization, and perceptual feature maps are obtained from contrast sensitivity formulations of retinal ganglion cells. The proposed quality estimator CSV is tested on the LIVE, the Multiply Distorted LIVE, and the TID 2013 databases, and it is always among the top two performing quality estimators in terms of at least ranking, monotonic behavior or linearity.

==> Preprint for ArXiv/fig_hist_v2.tex <==

\begin{figure}[htbp!]
\vspace{2.0mm}
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.8\linewidth, trim= 25mm 80mm 25mm 80mm]{Figs/hists_scatters/hist-live-dmos.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(a)LIVE-DMOS}}%\medskip
      \vspace{-0.20cm}

\end{minipage}
  \vspace{0.20cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.8\linewidth, trim= 25mm 80mm 25mm 80mm]{Figs/hists_scatters/hist-tid-mos.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(b) TID-MOS }}%\medskip
      \vspace{-0.20cm}

\end{minipage}
  \vspace{0.20cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.8\linewidth, trim= 25mm 80mm 25mm 80mm]{Figs/hists_scatters/hist-multi-dmos.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(c) MULTI-DMOS }}%\medskip
      \vspace{-0.20cm}

\end{minipage}



\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.8\linewidth, trim= 25mm 80mm 25mm 80mm]{Figs/hists_scatters/hist-live-ssim.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(d)LIVE-SSIM}}%\medskip
      \vspace{-0.20cm}
\end{minipage}
  \vspace{0.20cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.8\linewidth, trim= 25mm 80mm 25mm 80mm]{Figs/hists_scatters/hist-tid-ssim.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(e) TID-SSIM }}%\medskip
      \vspace{-0.20cm}
\end{minipage}
  \vspace{0.20cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.8\linewidth, trim= 25mm 80mm 25mm 80mm]{Figs/hists_scatters/hist-multi-ssim.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(f) MULTI-SSIM }}%\medskip
      \vspace{-0.20cm}
\end{minipage}

\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.8\linewidth, trim= 25mm 80mm 25mm 80mm]{Figs/hists_scatters/hist-live-iwssim.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(g)LIVE-IW-SSIM}}%\medskip
        \vspace{-0.20cm}
\end{minipage}
  \vspace{0.20cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.8\linewidth, trim= 25mm 80mm 25mm 80mm]{Figs/hists_scatters/hist-tid-iwssim.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(h) TID-IW-SSIM }}%\medskip
        \vspace{-0.20cm}
\end{minipage}
  \vspace{0.20cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.8\linewidth, trim= 25mm 80mm 25mm 80mm]{Figs/hists_scatters/hist-multi-iwssim.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(i) MULTI-IW-SSIM }}%\medskip
  \vspace{-0.20cm}
\end{minipage}


\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.8\linewidth, trim= 25mm 80mm 25mm 80mm]{Figs/hists_scatters/hist-live-fsimc.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(j)LIVE-FSIMc}}%\medskip
  \vspace{-0.20cm}  
  \end{minipage}
  \vspace{0.20cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.8\linewidth, trim= 25mm 80mm 25mm 80mm]{Figs/hists_scatters/hist-tid-fsimc.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(k) TID-FSIMc }}%\medskip
  \vspace{-0.20cm}
\end{minipage}
  \vspace{0.20cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.8\linewidth, trim= 25mm 80mm 25mm 80mm]{Figs/hists_scatters/hist-multi-fsimc.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(l) MULTI-FSIMc }}%\medskip
  \vspace{-0.20cm}

\end{minipage}


\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.8\linewidth, trim= 25mm 80mm 25mm 80mm]{Figs/hists_scatters/hist-live-csv.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(m)LIVE-CSV}}%\medskip
  \vspace{-0.20cm}
\end{minipage}
  \vspace{0.20cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.8\linewidth, trim= 25mm 80mm 25mm 80mm]{Figs/hists_scatters/hist-tid-csv.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(n) TID-CSV }}%\medskip
  \vspace{-0.20cm}
\end{minipage}
  \vspace{0.20cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.8\linewidth, trim= 25mm 80mm 25mm 80mm]{Figs/hists_scatters/hist-multi-csv.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(o) MULTI-CSV }}%\medskip
  \vspace{-0.20cm}  
\end{minipage}



\caption{Histograms of the objective quality estimates and the subjective scores.}
\label{fig:Histograms}
\vspace{-7.0mm}
\end{figure}


==> Preprint for ArXiv/fig_scatter_v2.tex <==

\begin{figure}[htbp!]
%\vspace{-15.0mm}

\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.9\linewidth, trim= 20mm 65mm 20mm 65mm]{Figs/hists_scatters/ssim_live.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(a)LIVE-SSIM}}%\medskip
  \vspace{-0.45cm}

\end{minipage}
 \vspace{0.2cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.9\linewidth, trim= 20mm 65mm 20mm 65mm]{Figs/hists_scatters/ssim_tid.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(b) TID-SSIM }}%\medskip
    \vspace{-0.45cm}

\end{minipage}
 \vspace{0.2cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.9\linewidth, trim= 20mm 65mm 20mm 65mm]{Figs/hists_scatters/ssim_multi.pdf}
  \vspace{0.03 cm}
  \centerline{\footnotesize{(c) MULTI-SSIM   } }%\medskip
    \vspace{-0.45cm}
\end{minipage}


\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.9\linewidth, trim= 20mm 65mm 20mm 65mm]{Figs/hists_scatters/iwssim_live.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(d)LIVE-IW-SSIM}}%\medskip
      \vspace{-0.45cm}
\end{minipage}
 \vspace{0.2cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.9\linewidth, trim= 20mm 65mm 20mm 65mm]{Figs/hists_scatters/iwssim_tid.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(e) TID-IW-SSIM }}%\medskip
      \vspace{-0.45cm}
\end{minipage}
 \vspace{0.2cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.9\linewidth, trim= 20mm 65mm 20mm 65mm]{Figs/hists_scatters/iwssim_multi.pdf}
  \vspace{0.03 cm}
  \centerline{\footnotesize{(f) MULTI-IW-SSIM   } }%\medskip
      \vspace{-0.45cm}
\end{minipage}


\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.9\linewidth, trim= 20mm 65mm 20mm 65mm]{Figs/hists_scatters/fsimc_live.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(g)LIVE-FSIMc}}%\medskip
      \vspace{-0.45cm}
\end{minipage}
 \vspace{0.2cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.9\linewidth, trim= 20mm 65mm 20mm 65mm]{Figs/hists_scatters/fsimc_tid.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(h) TID-FSIMc }}%\medskip
      \vspace{-0.45cm}
\end{minipage}
 \vspace{0.2cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.9\linewidth, trim= 20mm 65mm 20mm 65mm]{Figs/hists_scatters/fsimc_multi.pdf}
  \vspace{0.03 cm}
  \centerline{\footnotesize{(i) MULTI-FSIMc   } }%\medskip
      \vspace{-0.45cm}
\end{minipage}



\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.9\linewidth, trim= 20mm 65mm 20mm 65mm]{Figs/hists_scatters/csv_live.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(j)LIVE-CSV}}%\medskip
      \vspace{-0.45cm}
\end{minipage}
 \vspace{0.2cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.9\linewidth, trim= 20mm 65mm 20mm 65mm]{Figs/hists_scatters/csv_tid.pdf}
  \vspace{0.03cm}
  \centerline{\footnotesize{(k) TID-CSV }}%\medskip
      \vspace{-0.45cm}
\end{minipage}
 \vspace{0.2cm}
\hfill
\begin{minipage}[b]{0.28\linewidth}
  \centering
\includegraphics[width=0.9\linewidth, trim= 20mm 65mm 20mm 65mm]{Figs/hists_scatters/csv_multi.pdf}
  \vspace{0.03 cm}
  \centerline{\footnotesize{(l) MULTI-CSV   } }%\medskip
      \vspace{-0.45cm}
\end{minipage}


\caption{Scatter plots of the objective quality estimates and the subjective scores.}\vspace{-.5cm}
\label{fig:Scatter}
\vspace{-4.0mm}
\end{figure}


==> Preprint for ArXiv/parameters.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\tiny
\caption{The parameters in the proposed method \texttt{CSV}.}
\label{tab:param}
\begin{tabular}{|l|l|l|}
\hline
\textbf{CSV Block}                & Parameter & Value     \\ \hline
\multirow{5}{*}{\textbf{CIEDE}}   & $W$       & $[20,20]$ \\ \cline{2-3} 
                                  & $K_L$     & $1.0$     \\ \cline{2-3} 
                                  & $K_C$     & $1.0$     \\ \cline{2-3}
                                  & $K_H$     & $1.0$     \\ \cline{2-3}
                                   
                                  & $T$     & $20$     \\ \hline
\multirow{2}{*}{\textbf{CND}}     & $W$       & $[20,20]$ \\ \cline{2-3} 
                                  & $N$       & $11$      \\ \hline
\textbf{SD}                       & $W$       & $[20,20]$ \\ \hline
\multirow{2}{*}{\textbf{RGCD}}    & $W$       & $[20,20]$ \\ \cline{2-3} 
                                  & $\sigma$  & $50$      \\ \hline
\multirow{2}{*}{\textbf{Pooling}} & $A$       & $0.9$     \\ \cline{2-3} 
                                  & $P$       & $4$       \\ \hline
\end{tabular}
\end{table}

==> Preprint for ArXiv/tab_hist_dist_v3.tex <==

\begin{table*}[htbp!]%[htbp]
\vspace{-5.0mm}

\begin{adjustwidth}{-1.8cm}{}

  \centering
      \tiny
        \caption{Distributional difference between the subjective scores and the objective quality estimates.}

    \begin{tabular}{|c||c|c|c|c|c||c|c|c|c|c||c|c|c|c|c|}   \hline
    \multirow{2}[4]{*}{\textbf{Metric}} 
    
    & \multicolumn{5}{c||}{\textbf{Difference-LIVE}} & \multicolumn{5}{c||}{\textbf{Difference-TID}} & \multicolumn{5}{c|}{\textbf{Difference-Multi}} \\ \cline{2-16}     
    
          & \textbf{EMD}& \textbf{KL}& \textbf{JS}& \textbf{HI}& \textbf{L2}& \textbf{EMD}& \textbf{KL}& \textbf{JS}& \textbf{HI}& \textbf{L2}  & \textbf{EMD}& \textbf{KL}& \textbf{JS}& \textbf{HI}& \textbf{L2}    
          \\ \hline 

				\textbf{CSV} &\textbf{0.19} &\textbf{0.18} &\textbf{0.03} &\textbf{0.19} &\textbf{0.05}&\textbf{0.30}&\textbf{0.48}&\textbf{0.08}&\textbf{0.30}&\textbf{0.09} &\textbf{0.26}&\textbf{0.15}&\textbf{0.03}&\textbf{0.26}&\textbf{0.07} \\ \hline

	\textbf{FSIMc} &0.27 &0.29 &0.06 &0.27 &0.07&0.39&0.96&0.12&0.39&0.11 &0.42&0.51&0.10&0.42&0.12  \\ 


	\textbf{IW-SSIM} &0.30 &0.34 &0.07 &0.30 &0.07&0.50&1.67&0.19&0.50&0.18 &0.38&0.37&0.07&0.38&0.10  \\ 


	\textbf{SSIM} &0.28 &0.30 &0.06 &0.28 &0.07 &0.64&1.98&0.26&0.64&0.18 &0.38&0.41&0.08&0.38&0.10 \\ \hline

		

		
    \end{tabular}%
  \label{tab:hist_dist}
  \end{adjustwidth}{}

\end{table*} 



==> Preprint for ArXiv/tab_live_v2.tex <==


\begin{table}[htbp!]

  \centering
    \tiny
    \caption{Performance of the methods in the LIVE database.}

    \begin{tabular}{|c||c|c|c|c|c|c|}   \hline   
    
    
    
    \multirow{2}[3]{*}{\textbf{Sequence}} 
    


          & \textbf{Jp2k}& \textbf{JPEG}& \textbf{Wn}& \textbf{Gblur}& \textbf{FF}  & \textbf{All}   
          
 \\ \cline{2-7}


    & \multicolumn{6}{c|}{\textbf{Pearson (PLCC)}}               \\ \hline     
    
	\textbf{CSV} &\bf 0.983 &\bf 0.978 &\bf 0.986  &\textbf{0.971}  &0.949 &\textbf{0.967}  \\ 
	\textbf{$CSV_b$} &\bf 0.000&\bf 0.000&\bf 0.000& -0.007&-0.004&\bf -0.001  \\ 
	\textbf{$CSV_n$} &\bf 0.000&\bf 0.000&\bf 0.000& -0.007&-0.004&\bf -0.001  \\  
	\textbf{$CSV_e$} &-0.008&-0.014&-0.001&\bf 0.000&-0.002&-0.034  \\ \hline
	\textbf{CIEDE}  &-0.035&-0.025&-0.004&-0.028&-0.085&-0.051\\ 

	\textbf{CND}  &-0.028&-0.012&-0.020&-0.043&-0.084&-0.044\\ 

	\textbf{RGCD}  &-0.005 &-0.004 &\textbf{+0.002}  &-0.014  &-0.023 &-0.005 \\
	\textbf{SD}  &-0.021&-0.023&-0.030&\ -0.008&\textbf{+0.031}&-0.021   \\ 
	\textbf{RGCD$\cdot$SD}  &-0.002&-0.006&-0.009&\textbf{+0.006}&\bf +0.006&-0.003   \\ \hline
	
	

	\textbf{MSE} &-0.048&-0.043&-0.020&-0.098&-0.049&-0.055\\ 
	
	
  \textbf{SSIM} &-0.020&-0.020&-0.010&-0.031&\textbf{+0.007}&-0.022\\ 

  
  
  \textbf{MS-SSIM} &-0.020&-0.017&-0.008&-0.028&-0.001&-0.020\\ 


 \textbf{IW-SSIM} &-0.023&-0.019&-0.005&-0.014&+0.003&-0.015\\ 

 \textbf{CW-SSIM} &-0.056&-0.050&-0.037&-0.203&-0.114&-0.095\\ 


 \textbf{FSIMc} &-0.023&-0.029&-0.009& -0.015&+0.003&-0.018\\ 

 \textbf{PSNR-HA} 
&-0.001&-0.008&\textbf{0.000}&-0.023&+0.003&-0.008\\ \hline



  
 




    & \multicolumn{6}{c|}{\textbf{Spearman}}           \\ \hline    
 
 	\textbf{CSV} &\textbf{0.980}&0.960&\textbf{0.991}&0.973&0.937&0.959 \\ 
	\textbf{$CSV_b$} &\bf 0.000&0.000&\bf 0.000&-0.006&-0.006&-0.001  \\ 
	\textbf{$CSV_n$} &\bf 0.000&0.000&\bf 0.000&-0.006&-0.005&-0.001 \\  
	\textbf{$CSV_e$} &-0.003&-0.004&\bf +0.002&-0.008&+0.011&-0.011  \\  \hline
	\textbf{CIEDE}  &-0.011 &-0.002 &-0.007  &-0.034  &-0.117 &-0.060   \\ 
	
	\textbf{CND}  &-0.021 &-0.005 &-0.015 &-0.084  &-0.122  &-0.064     \\	

	\textbf{RGCD}  &-0.010 &-0.007 &-0.001  &-0.025  &-0.027 &-0.009   \\ 



	\textbf{SD}  &-0.026&-0.022&-0.024&-0.017&\textbf{+0.034}&-0.030 \\ 


	\textbf{RGCD$\cdot$SD}  &\textbf{+0.001}&0.000&\textbf{+0.002}&\textbf{+0.004}&+0.009&\textbf{+0.001}   \\ \hline
	 
 
 	\textbf{MSE} &-0.026 &-0.028 &\textbf{0.000} &-0.100 &-0.001 &-0.049 \\  
	
	  \textbf{SSIM} &0.000 &\textbf{+0.001} &-0.009 &-0.001 &\textbf{+0.036} &-0.009 \\ 
  \textbf{MS-SSIM} &0.000 &\textbf{+0.002} &-0.007 &0.000 &+0.031 &-0.007 \\ 

 \textbf{IW-SSIM} &-0.001 &0.000 &-0.010 &\textbf{+0.010} &+0.029 &\textbf{+0.001}  \\ 

 \textbf{CW-SSIM} &-0.034 &-0.017 &-0.008 &-0.117 &-0.052 &-0.056 \\

 \textbf{FSIMc} &\textbf{+0.001}&\textbf{+0.002}&-0.012&\textbf{+0.009}&\textbf{+0.033}&\textbf{+0.002}  \\ 

 \textbf{PSNRHA}  &-0.003&-0.001&+0.001&-0.011&+0.010&-0.013  \\ \hline





   








    & \multicolumn{6}{c|}{\textbf{Kendall}}       \\ \hline    
 

    \textbf{CSV} &\textbf{0.885} &0.840 &0.927 &0.868 &0.806 &0.834 
      \\ 
      
	\textbf{$CSV_b$} & \bf 0.000 &+0.002&0.000&-0.015&-0.010&-0.002  \\ 
	\textbf{$CSV_n$} & \bf 0.000 &+0.002&0.000&-0.014&-0.010&-0.002 \\  
	\textbf{$CSV_e$} &-0.008&-0.014& \bf +0.010&-0.022&+0.016&-0.022  \\  \hline    

	\textbf{CIEDE}  &-0.026 &-0.005 &-0.029 &-0.066  &-0.147  &-0.100  \\ 
	
	\textbf{CND}   &-0.050 &-0.013 &-0.058 &-0.132 &-0.154  &-0.106    \\

	
	\textbf{RGCD}   &-0.025 &-0.024 &-0.005 &-0.059  &-0.040  &-0.018  \\ 

	\textbf{SD}   &-0.065&-0.048&-0.076&-0.034&+0.056&-0.058  \\

	\textbf{RGCD$\cdot$SD}  &\textbf{+0.004}&0.000&\textbf{+0.010}&\textbf{+0.010}&+0.016&\textbf{+0.003}   \\ \hline
 
 	\textbf{MSE} &-0.060 &-0.059 &-0.002 &-0.164 &-0.015 &-0.085\\ 	
	  \textbf{SSIM} &0.000 &+0.003 &-0.032 &-0.010 &\textbf{+0.065} &-0.019\\  
  \textbf{MS-SSIM}  &-0.001 &\textbf{+0.008} &-0.023 &-0.004 &\textbf{+0.057} &-0.015\\ 
 \textbf{IW-SSIM} &-0.003 &\textbf{+0.006} &-0.034 &\textbf{+0.027} &+0.056 &\textbf{+0.004} \\
 

 \textbf{CW-SSIM} &-0.084 &-0.040 &-0.032 &-0.178 &-0.089 &-0.102 \\



 \textbf{FSIMc} &\textbf{+0.006}&\textbf{+0.012}&-0.041 &\textbf{+0.026}&\textbf{+0.063}&\textbf{+0.004}  \\ 

 \textbf{PSNRHA} &-0.008&-0.008&\bf +0.009&-0.028&+0.005&-0.029  \\ \hline



	









    \end{tabular}%
  \label{tab:LIVE_Results}
\vspace{-6.0mm}
\end{table} 


==> Preprint for ArXiv/tab_multi_v2.tex <==

\begin{table}[htbp!]

  \centering
    \tiny
    \caption{Performance of the methods in the MULTI database.}

    \begin{tabular}{|c||c|c|c|}   \hline   
    
    
    
    \multirow{2}[3]{*}{\textbf{Sequence}} 
    


          & \textbf{Blur+JPEG}& \textbf{Blur+Noise} & \textbf{All}   
          
 \\ \cline{2-4}


    & \multicolumn{3}{c|}{\textbf{Pearson (PLCC)}}               \\ \hline     
    

	\textbf{CSV} &\textbf{0.836}&\textbf{0.871}&\textbf{0.852}  \\ 
	\textbf{$CSV_b$} &0.000&\bf -0.001&-0.002  \\ 
	\textbf{$CSV_n$} &0.000&\bf -0.001&-0.002  \\  
	\textbf{$CSV_e$} &-0.029&-0.013&-0.024  \\ \hline
 	\textbf{CIEDE}  &-0.610&-0.212&-0.420\\ 
	\textbf{CND} &-0.493&-0.211&-0.359\\ 
	\textbf{RGCD}  &-0.057&-0.054&-0.057\\ 
	\textbf{SD}  &-0.011&-0.100&-0.074\\ 
	\textbf{RGCD$\cdot$SD} &\bf +0.015&\bf +0.015&\bf +0.016\\ \hline
	\textbf{MSE} &-0.107&-0.100&-0.110\\ 
  \textbf{SSIM} &-0.039&-0.037&-0.039\\  
  \textbf{MS-SSIM} &-0.043&-0.032&-0.049\\ 
 \textbf{IW-SSIM} &\textbf{+0.001}&-0.012&\bf 0.000\\
 \textbf{CW-SSIM} &-0.428&-0.495&-0.472\\ 
  \textbf{FSIMc} &-0.017&-0.053&-0.033\\ 
 \textbf{PSNR-HA} &\textbf{+0.001}&-0.067&-0.030\\ \hline

    & \multicolumn{3}{c|}{\textbf{Spearman}}           \\ \hline
 
    \textbf{CSV}&0.840&0.856&0.848       \\ 
	\textbf{$CSV_b$} &-0.001&-0.003&-0.002  \\ 
	\textbf{$CSV_n$} &0.000&-0.002&-0.002  \\ 
	\textbf{$CSV_e$} &-0.039&-0.015&-0.034  \\ \hline
	\textbf{CIEDE}  &-0.567&-0.256&-0.493\\ 
    \textbf{CND}  &-0.495&-0.312&-0.435\\ 
	\textbf{RGCD} &-0.062&-0.066&-0.064\\ 
	\textbf{BSD}  &-0.041&-0.135&-0.125\\ 
	\textbf{RGCD$\cdot$SD}  &+0.007&\textbf{+0.017}&+0.010\\ \hline
 	\textbf{MSE} &-0.178&-0.147&-0.171\\ 
	  \textbf{SSIM} &\textbf{+0.008}&\textbf{+0.019}&\textbf{+0.011}\\ 
  \textbf{MS-SSIM} &0.000&+0.006&-0.012\\	
 \textbf{IW-SSIM} &\textbf{+0.029}&\textbf{+0.037}&\textbf{+0.034}\\ 
  \textbf{CW-SSIM} &-0.201&-0.224&-0.218\\ 
 \textbf{FSIMc} &\textbf{+0.013}&+0.008&\textbf{+0.014}\\ 
 \textbf{PSNRHA}  &-0.098&-0.118&-0.105\\ \hline


    & \multicolumn{3}{c|}{\textbf{Kendall}}       \\ \hline    
     \textbf{CSV} &0.646&0.665&0.655       \\ 
	\textbf{$CSV_b$} &-0.002&-0.005&-0.004  \\ 
	\textbf{$CSV_n$} &-0.001&-0.005&-0.003  \\ 
	\textbf{$CSV_e$} &-0.046&-0.012&-0.036  \\   \hline 
	\textbf{CIEDE}  &-0.460&-0.226&-0.405\\ 
	\textbf{CND}   &-0.410&-0.275&-0.367\\ 
	\textbf{RGCD}   &-0.068&-0.066&-0.069\\ 
	\textbf{SD}   &-0.050&-0.137&-0.126\\ 
	\textbf{RGCD$\cdot$SD}  &\textbf{+0.006}&\textbf{+0.017}&+0.013\\ \hline
 	\textbf{MSE} &-0.169&-0.136&-0.155\\ 
	  \textbf{SSIM} &+0.005&\textbf{+0.021}&\textbf{+0.014}\\ 
  \textbf{MS-SSIM}  &-0.003&+0.009&-0.011\\ 
 \textbf{IW-SSIM} &\textbf{+0.036}&\textbf{+0.043}&\textbf{+0.046}\\ 
  \textbf{CW-SSIM} &-0.181&-0.204&-0.198\\ 
 \textbf{FSIMc} &\textbf{+0.013}&+0.004&\textbf{+0.017}\\ 
 \textbf{PSNRHA} &-0.094&-0.111&-0.096\\ \hline
    \end{tabular}%
  \label{tab:Multi_Results}
\end{table} 


==> Preprint for ArXiv/tab_sign_v3.tex <==

%
%\begin{table*}[htbp!]                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         
%\centering                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                
%    \tiny
%    \caption{ITU-T Rec. P.1401 Statistical significance test results}
%
%\begin{tabular}{|c|c|c|c|c|c|}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            
%\hline                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    
% & CSV & FSIMc & IWSSIM & MSSSIM & PSNRHA \\                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              
%\hline                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    
%CSV & 0  0  0  0  0  0  0  0  0 & 1  0  0  1  0  0  0  0  0 & 1  0  0  1  1  1  0  0  0 & 1  0  0  1  1  1  1  0  0 & 1  1  1  0  1  0  0  1  1 \\                                                                                                                                                                                                                                                                                                                                                                                                                                                                        
%\hline                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    
%FSIMc & 1  0  0  1  0  0  0  0  0 & 0  0  0  0  0  0  0  0  0 & 0  0  0  0  1  1  0  0  0 & 0  1  0  0  1  1  0  0  0 & 1  1  1  0  1  0  0  1  1 \\                                                                                                                                                                                                                                                                                                                                                                                                                                                                      
%\hline                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    
%IWSSIM & 1  0  0  1  1  1  0  0  0 & 0  0  0  0  1  1  0  0  0 & 0  0  0  0  0  0  0  0  0 & 0  1  0  0  0  0  1  1  0 & 1  1  1  0  1  1  0  1  1 \\                                                                                                                                                                                                                                                                                                                                                                                                                                                                     
%\hline                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    
%MSSSIM & 1  0  0  1  1  1  1  0  0 & 0  1  0  0  1  1  0  0  0 & 0  1  0  0  0  0  1  1  0 & 0  0  0  0  0  0  0  0  0 & 1  1  0  0  1  1  0  1  1 \\                                                                                                                                                                                                                                                                                                                                                                                                                                                                     
%\hline                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    
%PSNRHA & 1  1  1  0  1  0  0  1  1 & 1  1  1  0  1  0  0  1  1 & 1  1  1  0  1  1  0  1  1 & 1  1  0  0  1  1  0  1  1 & 0  0  0  0  0  0  0  0  0 \\                                                                                                                                                                                                                                                                                                                                                                                                                                                                     
%\hline                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    
%\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             
%\vspace{-3.0mm}
%\label{tab:sign}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   
%\end{table*} 


\begin{table*}[htbp!]                                                                                                                                    
\centering                                                                                                                                           
\tiny
\begin{tabular}{|c|c|c|c|c|}                                                                                                                       
\hline                                                                                                                                               
 & CSV & FSIMc & IWSSIM  & SSIM \\                                                                                                           
\hline                                                                                                                                               
CSV & 0  0  0  0  0  0  0  0  0 & 1  0  0  1  0  0  0  0  0 & 1  0  0  1  1  1  0  1  0  & 1  1  0  1  1  1  0  0  0 \\ \hline
FSIMc & 1  0  0  1  0  0  0  0  0 & 0  0  0  0  0  0  0  0  0 & 0  0  0  0  1  1  0  0  0  & 0  1  0  1  1  1  0  0  0 \\                                                                                                                                                
IWSSIM & 1  0  0  1  1  1  0  1  0 & 0  0  0  0  1  1  0  0  0 & 0  0  0  0  0  0  0  0  0  & 0  1  0  1  1  1  0  0  0 \\                                                                                                                                               SSIM & 1  1  0  1  1  1  0  0  0 & 0  1  0  1  1  1  0  0  0 & 0  1  0  1  1  1  0  0  0  & 0  0  0  0  0  0  0  0  0 \\  
\hline                                                                                                                                               
\end{tabular}                                                                                                                                        
\caption{ITU-T Rec. P.1401 statistical significance test results.}                                                                                    
\label{tab:sign}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   
\vspace{-10.0mm}
\end{table*} 

==> Preprint for ArXiv/tab_tid13_v2.tex <==
\begin{table*}[htbp!]
\begin{adjustwidth}{-3.5cm}{}

  \centering
    \tiny
    \caption{Performance of the methods in the TID 2013 database.}
    \begin{tabular}{|c||c|c|c|c|c|c|c||c|c|c|c|c|c|c|}   \hline

%    \multirow{2}[3]{*}{Sequence} & \multicolumn{7}{|c|}{Spearman}  \\ %\cline{2-8}
%          & Noise& Actual& Simple& Exotic& New  & Color &Full  \\ \hline

    \multirow{2}[3]{*}{\textbf{Sequence}} 
    
    & \multicolumn{7}{c||}{\textbf{Spearman (SCC)}}     & \multicolumn{7}{c|}{\textbf{Kendall (KCC)}}  \\ \cline{2-15} 
    
    
    
          & \textbf{Noise}& \textbf{Actual}& \textbf{Simple}& \textbf{Exotic}& \textbf{New}  & \textbf{Color} &\textbf{Full}  
          & \textbf{Noise}& \textbf{Actual}& \textbf{Simple}& \textbf{Exotic}& \textbf{New}  & \textbf{Color} &\textbf{Full}  
          
          
          \\ \hline  



	\textbf{CSV} &0.849 &0.880 &0.924 &0.812 &\textbf{0.898}  &\textbf{0.888}  &\textbf{0.845}
	 &0.665 &0.710 &0.758 &0.605 &\textbf{0.724}  &\textbf{0.713}  &\textbf{0.654}  \\ 

		\textbf{$CSV_b$} &+0.006&+0.003&-0.003&-0.003&\bf +0.013&\bf +0.021&\bf +0.003 
		&+0.006&+0.003&-0.007&-0.004&\bf +0.016&\bf +0.028&\bf +0.004 \\ 
		\textbf{$CSV_n$} &+0.007&+0.004&-0.003&-0.006&+\bf 0.012&\bf +0.021&+0.002 
		&+0.007&+0.004&-0.008&-0.007&\bf +0.015&\bf +0.028&+0.002 \\ 
		\textbf{$CSV_e$} &-0.008&0.000&+0.012&-0.042&-0.049&-0.081&-0.048
		 &-0.008&0.000&+0.021&-0.044&-0.053&-0.093&-0.049 \\ \hline
		\textbf{CIEDE} &-0.019&-0.016&-0.115&-0.416&-0.145&-0.026&-0.229
	     &-0.032&-0.034&-0.152&-0.337&-0.181&-0.058&-0.211\\ 
	\textbf{CND} &-0.068&-0.066&-0.223&-0.505&-0.136&-0.044&-0.267
	&-0.082&-0.088&-0.251&-0.381&-0.164&-0.071&-0.237\\ 
	\textbf{RGCD} &+0.023&+0.011&+0.009&-0.089&+0.005&-0.005&-0.030
	&+0.023&+0.005&+0.020&-0.053&+0.010&-0.009&-0.015\\ 
	\textbf{SD} &-0.287&-0.225&-0.174&-0.227&-0.289&-0.370&-0.301
	&-0.277&-0.244&-0.217&-0.191&-0.285&-0.348&-0.267\\ 
	\textbf{RGCD$\cdot$SD}&-0.024&-0.017&-0.001&-0.005&-0.101&-0.138&-0.040
	&-0.024&-0.021&0.000&+0.010&-0.105&-0.141&-0.032\\ \hline
	\textbf{FSIMc} &+0.052&+0.034&+0.022&\textbf{+0.028}&-0.110&-0.113&\textbf{+0.005}
	&+0.057&+0.032&+0.034&\textbf{+0.046}&-0.112&-0.121&\textbf{+0.012}\\ 
    \textbf{PSNR-HA} &\textbf{+0.073}&\textbf{+0.057}&\textbf{+0.027}&+0.012&-0.197&-0.256&-0.026
    &\textbf{+0.094}&\textbf{+0.076}&\textbf{+0.059}&+0.018&-0.182&-0.236&-0.010\\ 
    \textbf{PSNR-HMA} &\textbf{+0.065}&\textbf{+0.053}&+0.012&+0.001&-0.160&-0.214&-0.032
    &\textbf{+0.079}&\textbf{+0.066}&+0.026&+0.004&-0.151&-0.206&-0.022\\ 
	\textbf{FSIM} &+0.047&+0.030&\textbf{+0.023}&\textbf{+0.031}&-0.249&-0.323&-0.044
	&+0.050&+0.026&\textbf{+0.036}&\textbf{+0.049}&-0.200&-0.261&-0.024\\ 
	\textbf{MS-SSIM} &+0.023&+0.006&-0.019&\textbf{+0.029}&-0.267&-0.322&-0.058
	&+0.014&-0.012&-0.037&\textbf{+0.042}&-0.229&-0.258&-0.046\\ 
	\textbf{IW-SSIM}
&+0.021&+0.006&-0.013&\bf +0.028&-0.279&-0.339&-0.067
&+0.013&-0.009&-0.028&+0.038&-0.248&-0.289&-0.056\\ 
	\textbf{PSNRc} &-0.080&-0.077&-0.049&-0.249&-0.121&-0.154&-0.158
	&-0.103&-0.114&-0.069&-0.213&-0.148&-0.178&-0.158\\ 
	\textbf{VSNR} &+0.019&+0.001&-0.012&-0.105&-0.309&-0.376&-0.164
	&+0.010&-0.019&-0.027&-0.086&-0.286&-0.335&-0.146\\ 
	\textbf{PSNR-HVS} &\textbf{+0.067}&\textbf{+0.045}&\textbf{+0.025}&-0.211&-0.251&-0.329&-0.191
	&\textbf{+0.089}&\textbf{+0.055}&\textbf{+0.050}&-0.170&-0.207&-0.265&-0.146\\ 
	\textbf{PSNR} &-0.028&-0.055&-0.011&-0.215&-0.279&-0.349&-0.206
	&-0.042&-0.086&-0.013&-0.180&-0.251&-0.298&-0.184\\ 
	\textbf{SSIM} &-0.092&-0.092&-0.087&-0.180&-0.318&-0.382&-0.208
	&-0.114&-0.133&-0.130&-0.150&-0.301&-0.331&-0.190 \\ 
	\textbf{NQM} &-0.013&-0.023&-0.049&-0.222&-0.272&-0.346&-0.210
	&-0.024&-0.044&-0.077&-0.193&-0.241&-0.305&-0.188\\ 
	\textbf{PSNR-HVS-M} &+0.056&+0.037&+0.013&-0.247&-0.251&-0.331&-0.220
	&+0.067&+0.038&+0.021&-0.202&-0.206&-0.273&-0.172\\ 
	\textbf{VIFP} &-0.066&-0.065&-0.027&-0.254&-0.306&-0.379&-0.237
	&-0.078&-0.089&-0.044&-0.199&-0.273&-0.320&-0.197\\ 
	\textbf{WSNR}&+0.030&+0.016&+0.008&-0.389&-0.251&-0.329&-0.265
	&+0.030&+0.007&+0.014&-0.308&-0.209&-0.277&-0.207\\ \hline
    \end{tabular}%
  \label{tab:TID_Results}
\vspace{-1.0mm}
\end{adjustwidth}{}
\end{table*} 


